Task Graph Transformations for Latency Tolerance

The Integrative Model for Parallelism (IMP) derives a task graph from a higher level description of parallel algorithms. In this note we show how task graph transformations can be used to achieve latency tolerance in the program execution. We give a formal derivation of the graph transformation, and show through simulation how latency tolerant algorithms can be faster than the naive execution in a strong scaling scenario.

==> hiding.tex <==
% -*- latex -*-
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% This text file is part of the theory writeup on the
%%%% Integrative Model for Parallelism,
%%%% copyright Victor Eijkhout (eijkhout@tacc.utexas.edu) 2014-6
%%%%
%%%% hiding.tex : include file for report IMP-06
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Orchestrating data transfer}

%\begin{figure}[ht]
  \begin{wrapfigure}{r}{2in}
    \includegraphics[scale=.04]{task-send1}
    \caption{Depiction of task $(k_1,q)$ sending data to $(k_2,p)$}
    \label{fig:tasksend1}
  \end{wrapfigure}
%\end{figure}
%
In figure~\ref{fig:tasksend1} we depict the logical structure of data
transfer: kernel~$k_1$ produces data (specifically, in processor~$q$), which is needed in
kernel~$k_2$ (specifically, in processor~$q$).
(While the picture makes the kernel tasks look synchronized, that is,
all tasks in $k_1$ happening before~$k_1$, this need not be the case
in practice.)

Actually realizing this conceptual picture in practice is not
trivial. We know that kernel~$k_2$ takes a certain object as input, so
the easiest implementation posts both the sends and receives for that
object as a first step in~$k_2$. This is depicted in
figure~\ref{fig:tasksend2}. However, we would like to post the
send/receive operations earlier, so that we can take advantage of
possible offloaded communication.

%\begin{figure}[ht]
  \begin{wrapfigure}{r}{2in}
\includegraphics[scale=.04]{task-send2}
  \caption{Data transfer as part of $k_2$}
  \label{fig:tasksend2}
\end{wrapfigure}
%\end{figure}
%
The optimized solution is then that the descriptors for the
send/receive operations are moved from $k_2$ which creates them, to
$k_1$ where can can earliest be executed. This means that the transfer
can overlap with any intervening kernel~$k_3$. It also means that the
space available for $k_3$ is diminished by buffer space for the
$k_1\rightarrow k_2$ transfer. See figure~\ref{fig:tasksend3}.

\begin{figure}[ht]
\includegraphics[scale=.04]{task-send3}
  \caption{Buffer space detracts from available space for intervening kernel~$k_3$}
  \label{fig:tasksend3}
\end{figure}

\subsection{Overlap}

\begin{figure}[ht]
  \includegraphics[scale=.5]{pipelineprods}
  \caption{Matrix-vector and vector-vector inner product in the kernel
    structure of pipelined CG}
  \label{fig:pipelineprods}
\end{figure}

We analyze the task graph to find operations that can potentially
overlap. For instance, in pipelined Conjugate Gradients~\cite{IMP-17}
the matrix-vector product and one inner product are seen to be
causally unrelated, hence overlappable; figure~\ref{fig:pipelineprods}.

Such an analysis is NP-complete in the general
case~\cite{Taylor:syncNP}, but becomes very efficient in the
parallelism model of IMP.


==> sync.tex <==
% -*- latex -*-
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%
%%%% This text file is part of the theory writeup on the
%%%% Integrative Model for Parallelism,
%%%% copyright Victor Eijkhout (eijkhout@tacc.utexas.edu) 2014-6
%%%%
%%%% sync.tex : include file for IMP-06
%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Once we have a task graph we have to worry about how to execute it.
In this section we give a rigorous definition of synchronization between processors
as it is induced by the task graph, and we will analyze execution behaviour
of the processors in terms of synchronization.

\subsection{Definition of synchronization}

The following definition of a synchronization point
makes immediate sense in the context of message passing:
\begin{definition}
  For a task $t\in T$ we define a task~$t'$ as a \indexterm{synchronization point} if
  $t'$~is an immediate predecessor on another processor:
  \[ t\in C_p \wedge t'<t \wedge t'\in C_{p'} \wedge p\not=p'. \]
\end{definition}
A synchronization point in MPI corresponds to a process that sends a message; in a shared memory task
graph it corresponds to a child task.

Using synchronization points we arrive at the concept of \emph{local
  computations}\index{local computation!definition of}: sets of tasks
$L\subset T$ that can be executed without synchronization, except for
possibly an initial synchronization. 

\begin{definition}
  Given a set of tasks $L\subset T$, we define its base~$B_L$ as
  \[ B = \{ t\in L\colon \pred(t)\not\subset L\}. \]
\end{definition}

The base of a subset~$L$ consists of the set of tasks with synchronization points.

\begin{definition}
  \label{def:localcomp}
  We call a two-parameter covering $\{L_{k,p}\}_{k,p}$ of~$T$ 
  a set of \emph{local computations} if
  \begin{enumerate}
  \item the $p$ index corresponds to the division in processors:
    \[ C_p = \cup_k L_{k,p}.  \]
  \item the $k$ index corresponds to the partial ordering on tasks:
    the sets $L_k=\cup_p L_{k,p}$ satisfy
    \[ t\in L_k \wedge t'<t \Rightarrow t'\in L_{k}\cup L_{k-1}\cup\cdots \]
  \item the synchronization points synchronize only with previous levels:
    \[ t\in L_{k,p}\wedge t'<t \wedge t'\not\in C_p \Rightarrow t'\in L_{k-1}\cup L_{k-2}\cup\cdots \]
    or
    \begin{equation}
      \pred(B_{k,p})-C_p\subset L_{k-1}\cup L_{k-2}\cup\cdots
      \label{eq:Lpred}
    \end{equation}
  \end{enumerate}
\end{definition}

\begin{theorem}
  For a given $k$, all $L_{k,p}$ can be executed independently.
\end{theorem}
\begin{proof}
  All predecessors that are in a different processor are also
  in a previous level.
\end{proof}

We illustrate this in figure~\ref{fig:LBs}.
\begin{figure}
  \hbox{%
    (a): \includegraphics[scale=.05]{LB1}
    (b): \includegraphics[scale=.05]{LB2}
    (c): \includegraphics[scale=.05]{LB3}
  }
  \caption{Three cases of L/B relations}
  \label{fig:LBs}
\end{figure}
Case (a) is the normal single step grid update, much like our 
motivating example.
Case (b) shows that for a second update we would need a point
on the same $k$-level, so this is not a well-formed local computation
by the above definition.
Case (c) shows how this is solved by transferring a larger halo,
and computing one point redundantly.

\subsection{Execution and synchronization}

At this point we should say something about synchronization.
The easiest way to visualize execution of local computations (in the above
definition) is to imagine a global synchronization point after each level.
This reduces our model to BSP~\cite{Valiant:1990:BSP}. However, this is overly restrictive.
Tasks in $L_{k,p}$ can start execution when their synchronization points in~$L_{k-1},L_{k-2},\ldots$
have executed. This means that local computations in different $k$-levels can be
active simultaneously.

In fact, if $\pred\bigl(B_{k,p}\bigr)$ has elements in $L_{k',p'}$, it is quite
possible for $L_{k',p'}$ not to have finished execution when $L_{k,p}$ starts.
Conversely, tasks in $L_{k,p}-B_{k,p}$ can execute before all of $B_{k,p}$
finishes. Thus, we arrive at a conception of a local computation that produces
streaming output and accepts streaming input during execution. This is a first 
interpretation of the concept of overlapping communication and computation.

We can now define the \indexterm{granularity} of a computation:
\begin{definition}
  The granularity of a computation $L_{k,p}$ is
  \[ g = \min_{k,p} |L_{k,p}|. \]
\end{definition}

We can also give a sufficient condition for overlap of communication and computation.
\begin{theorem}
  If we have the more restrictive condition (compared to equation~\eqref{eq:Lpred})
  \[ \pred(B_{k,p})-C_p\subset L_{k-2}\cup \cdots \]
  for all $k,p$, the communication can be overlapped with computation.
\end{theorem}
\begin{proof}
  All sends for level $k$ can be initiated at level $k-2$, so they can overlap
  with the computation of level~$k-1$.
\end{proof}


